Measuring the Leakage and Exploitability of Authentication Secrets in Super-apps: The WeChat Case

We conduct a large-scale measurement of developers' insecure practices leading to mini-app to super-app authentication bypass, among which hard-coding developer secrets for such authentication is a major contributor. We also analyze the exploitability and security consequences of developer secret leakage in mini-apps by examining individual super-app server-side APIs. We develop an analysis framework for measuring such secret leakage, and primarily analyze 110,993 WeChat mini-apps, and 10,000 Baidu mini-apps (two of the most prominent super-app platforms), along with a few more datasets to test the evolution of developer practices and platform security enforcement over time. We found a large number of WeChat mini-apps (36,425, 32.8%) and a few Baidu mini-apps (112) leak their developer secrets, which can cause severe security and privacy problems for the users and developers of mini-apps. A network attacker who does not even have an account on the super-app platform, can effectively take down a mini-app, send malicious and phishing links to users, and access sensitive information of the mini-app developer and its users. We responsibly disclosed our findings and also put forward potential directions that could be considered to alleviate/eliminate the root causes of developers hard-coding the app secrets in the mini-app's front-end code.

==> tables/cloudanalysis.tex <==
\begin{table}[H]
\centering
\begin{tabular}{lr}
\toprule
\textbf{\textcolor{brown}{Usage type}} & {Total miniapps} \\
\midrule
\rowcolor{lavender}
\# miniapps & 36,425 \\
\# miniapps with cloud base & 254 \\
\rowcolor{lavender}
\# miniapps with cloud functions & 202 \\
% \# distinct cloud functions & 992 \\
\# database usage & 179 \\
\rowcolor{lavender}
\# database collections & 534 \\
\bottomrule
\end{tabular}
    \caption{Analysis on the usage of cloud base in the miniapps\mm{Supraja - do you refer to this?}} %
    \label{tab:cloud-base-stats}
\end{table}


==> tables/visitsource.tex <==
\begin{table}[H]
\begin{tabular}{ |l|l| }
  \hline
  \multicolumn{2}{|c|}{Miniapp Visit Sources} \\
  \hline
  1 & The list of recently used Mini Programs \\
  2 & Search \\
  3 & Chat \\
  4 & Scan of QR code \\
  5 & Homepage of an Official Account \\
  6 & Drop-down panel on the Chat tab \\
  7 & Home screen of the device \\
  8 & Homepage of a Mini Program \\
  9 & Mini Programs Nearby \\
  11 & Message template \\
  13 & Menu of an Official Account \\
  14 & Share from an app \\
  15 & Payment completion page \\
  16 & Press and hold on a QR code \\
  17 & QR code in My Posts \\
  18 & Official Account article \\
  19 & Wallet \\
  20 & Cards \& Offers \\
  21 & Cards \& Offers in a Mini Program \\
  22 & Other Mini Programs \\
  23 & Response of other Mini Programs \\
  24 & Applicable Stores in Cards \& Offers \\
  25 & Quick entry to the search box \\
  26 & Customer service message in a Mini Program \\
  27 & Sent by an Official Account \\
  29 & Recently Used in the task bar \\
  30 & Press and hold the dote menu in the Mini Program \\
  31 & Wi-Fi connection success screen \\
  32 & Public Services \\
  33 & An ad on WeChat \\
  34 & Other mobile apps \\
  35 & Discover > Mini Programs > My Mini Programs \\
  36 & My Mini Programs in the task bar \\
  10 &  Other \\
  \hline
\end{tabular}
 \caption{Miniapp visit source as per documentation} %
     \label{tab:cloud-base-stats}
\vspace{100pt} 
\end{table}
